BAM-DETR: Boundary-Aligned Moment Detection Transformer for Temporal Sentence Grounding in Videos

Temporal sentence grounding aims to localize moments relevant to a language description. Recently, DETR-like approaches achieved notable progress by predicting the center and length of a target moment. However, they suffer from the issue of center misalignment raised by the inherent ambiguity of moment centers, leading to inaccurate predictions. To remedy this problem, we propose a novel boundary-oriented moment formulation. In our paradigm, the model no longer needs to find the precise center but instead suffices to predict any anchor point within the interval, from which the boundaries are directly estimated. Based on this idea, we design a boundary-aligned moment detection transformer, equipped with a dual-pathway decoding process. Specifically, it refines the anchor and boundaries within parallel pathways using global and boundary-focused attention, respectively. This separate design allows the model to focus on desirable regions, enabling precise refinement of moment predictions. Further, we propose a quality-based ranking method, ensuring that proposals with high localization qualities are prioritized over incomplete ones. Experiments on three benchmarks validate the effectiveness of the proposed methods. The code is available at https://github.com/Pilhyeon/BAM-DETR.

==> tables/table_4.tex <==

\begin{table}
\centering
\footnotesize
\setlength{\tabcolsep}{0pt}
\begin{threeparttable}
\begin{tabularx}
{\linewidth}
{@{\hspace{1mm}}p{2.4cm}p{1.4cm}<{\centering}p{1.4cm}<{\centering}p{1.4cm}<{\centering}p{1.4cm}<{\centering}p{1.4cm}<{\centering}}
\toprule
Method & R1@0.3 & R1@0.5 & R1@0.7 & mIoU \\
\midrule
2D-TAN~\cite{zhang20202d-tan} & 40.01 & 27.99 & 12.92 & 27.22 \\
VSLNet~\cite{zhang2020vslnet} & 35.54 & 23.54 & 13.15 & 24.99 \\
M-DETR~\cite{lei2021qvhighlights} & 37.97 & 24.67 & 11.97 & 25.49 \\
QD-DETR\tnote{\ddag}~\cite{moon2023qd-detr} & 52.39 & 36.77 & 21.07 & 35.76 \\
UniVTG~\cite{lin2023univtg}  & 51.44 & 34.97 & 17.35 & 33.60 \\
MomentDiff\tnote{\ddag}~\cite{li2023momentdiff} & 46.64 & 28.92 & 12.37 & 30.36 \\
\cmidrule{1-5}
{\ours} & \textbf{56.69} & \textbf{41.54} & \textbf{26.77} & \textbf{39.31} \\
\bottomrule
\end{tabularx}
\vspace{0.5mm}
\hspace{0.3mm}
\tnote{\ddag}reproduced by official codebase
\end{threeparttable}
\vspace{-2.9mm}
\caption{Results on the TACoS test split.}
\label{tab:tacos}
\end{table}

==> tables/table_7_tmp.tex <==

\newcommand{\TableAblationNumQueries}{
    \toprule
    
     & \multicolumn{2}{c}{R1} & & \multicolumn{3}{c}{mAP} \\
    \cline{2-3} \cline{5-7}    
    \vspace{-0.45cm}$M$    &@0.5 &@0.7 & &@0.5 &@0.75 &Avg. \\
    \midrule
        5 & 62.19  & 49.03  & & 62.26 & 46.50 & 45.18  \\
        \rowcolor{defaultcolor}
        10 & 65.10  & 51.61  & & 65.41 & 48.56 & 47.61  \\
        15 & 65.48  & 50.32  & & 65.34 & 49.77 & 48.23  \\
        20 & 65.23  & 51.61  & & 64.56 & 49.40 & 48.01  \\
    \bottomrule
}


\newcommand{\TableAblationBoundaryFeat}{
    \toprule
    
      & \multicolumn{2}{c}{R1} & & \multicolumn{3}{c}{mAP} \\
    \cline{2-3} \cline{5-7}    
    \vspace{-0.45cm}Memory    & @0.5 & @0.7 & & @0.5 & @0.75 & Avg. \\
    \midrule
        plain & 63.74  & 49.68  & & 64.10 & 47.74 & 46.21  \\
        sensitive & 63.81  & 49.87  & & 65.08 & 46.62 & 46.34  \\
        \rowcolor{defaultcolor}
        merged & 65.10  & 51.61  & & 65.41 & 48.56 & 47.61  \\
    \bottomrule
}


\newcommand{\TableAblationNumBoundaryPoint}{
    \toprule
    
      & \multicolumn{2}{c}{R1} & & \multicolumn{3}{c}{mAP} \\
    \cline{2-3} \cline{5-7}    
    \vspace{-0.45cm}$K$    & @0.5 & @0.7 & & @0.5 & @0.75 & Avg. \\
    \midrule
        1 (fixed) & 63.23  & 48.32  & & 63.53 & 46.42 & 45.17  \\
        1 & 64.32  & 49.87  & & 65.01 & 48.72 & 47.14  \\
        \rowcolor{defaultcolor}
        3 & 65.10  & 51.61  & & 65.41 & 48.56 & 47.61  \\
        5 & 64.90  & 50.45  & & 65.38 & 47.58 & 46.70  \\
    \bottomrule
}


\newcommand{\TableAblationQualityInput}{
    \toprule
    
     & & & \multicolumn{2}{c}{R1} & & & \multicolumn{3}{c}{mAP} \\
    \cline{4-5} \cline{7-9}    
    \vspace{-0.45cm}$\mathbf{C}_p$  & \vspace{-0.45cm}$\mathbf{C}_s$ & \vspace{-0.45cm}$\mathbf{C}_e$ & @0.5 & @0.7 & & @0.5 & @0.75 & Avg. \\
    \midrule
        \cmark &  &  & 62.97  & 49.03  & & 64.44 & 47.50 & 46.26  \\
         & \cmark &  & 64.39  & 50.71  & & 64.60 & 47.69 & 46.66  \\
         &  & \cmark & 64.58  & 49.23  & & 64.38 & 47.85 & 46.71  \\
        \rowcolor{defaultcolor}
        \cmark & \cmark & \cmark & 65.10  & 51.61  & & 65.41 & 48.56 & 47.61  \\
    \bottomrule
}



\newcommand{\TableAblationAttn}{
    \toprule
    
    Anchor & Boundary & \multicolumn{2}{c}{R1} & & \multicolumn{3}{c}{mAP} \\
    \cline{3-4} \cline{6-8}    
    query  & query & @0.5 & @0.7 & & @0.5 & @0.75 & Avg. & & \vspace{-0.45cm}FLOPs & & \vspace{-0.45cm}Params\\
    \midrule
        \multicolumn{2}{c}{Global (shared)} & 62.26  & 49.03  & & 62.63 & 45.90 & 44.18 & & 0.71G & & 8.2M \\
        Global & Global & 63.61  & 49.81  & & 64.11 & 45.38 & 44.54 & & 0.72G & & 11.5M \\
        \rowcolor{defaultcolor}
        Global & Focused & 63.74  & 49.68  & & 64.10 & 47.74 & 46.21  & & 0.65G &  & 9.5M \\
        Focused & Focused & 62.48  & 49.16  & & 63.90 & 47.31 & 45.87  & & 0.62G & & 7.6M \\
    \bottomrule
}




\begin{table*}[t]
    % \vspace{-.4em}
    \vspace{-2mm}
    \caption{Ablative experiments on QVHighlights. Default settings are marked \colorbox{defaultcolor}{gray}.
    }
    \centering
    %#################################################
    \captionsetup[subfloat]{labelfont=scriptsize,textfont=scriptsize}
    \subfloat[
    Number of predictions
    \label{tab:num_queries}
    ]{
    \centering
    \begin{minipage}[t]{0.3\linewidth}{
    \begin{center}
    \tablestyle{1pt}{1.1}
    \scriptsize
    {
    \begin{tabularx}{0.92\linewidth}{p{0.5cm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{1.0mm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{1.0mm}}
        \TableAblationNumQueries
    \end{tabularx}
    }
    \end{center}
    }
    \end{minipage}
    }
    % \hspace{0.5em}
    %#################################################
    \subfloat[
    \scriptsize
    Choice of memory features
    \label{tab:boundary_features}
    ]{
    \begin{minipage}[t]{0.337\linewidth}{
    \begin{center}
    \tablestyle{1pt}{1.1}
    \scriptsize
    {
    \begin{tabularx}{0.92\linewidth}{p{1.3cm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{1.0mm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{1.0mm}}
        \TableAblationBoundaryFeat
    \end{tabularx}
    }
    \end{center}
    }
    \end{minipage}
    }
    % \hspace{0.5em}
    %#################################################
    \subfloat[
    \scriptsize
    Number of boundary points
    \label{tab:num_boundary_points}
    ]{
    \begin{minipage}[t]{0.325\linewidth}{
    \begin{center}
    \tablestyle{1pt}{1.1}
    \scriptsize
    {
    \begin{tabularx}{0.92\linewidth}{p{1.1cm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{1.0mm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{1.0mm}}
        \TableAblationNumBoundaryPoint
    \end{tabularx}
    }
    \end{center}
    }
    \end{minipage}
    }\\
    % \vspace{-0.5em}
    % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %#################################################
       \subfloat[
    \scriptsize
    Query choices for quality prediction
    \label{tab:quality_input}
    ]{
    \centering
    \begin{minipage}[!b]{0.4\linewidth}{
    \begin{center}
    \tablestyle{1pt}{1.1}
    \scriptsize
    {
    \begin{tabularx}{0.92\linewidth}{p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{1.0mm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{1.0mm}}
        \TableAblationQualityInput
    \end{tabularx}
    }
    \end{center}
    }
    \end{minipage}
    % \hspace{0.5em}
    }%#################################################
    \subfloat[
    \scriptsize
    Combinations of attention layers for updating pathways
    \label{tab:attn_combination}
    ]{
    \centering
    \begin{minipage}[b]{0.59\linewidth}{
    \begin{center}
    \tablestyle{1pt}{1.1}
    \scriptsize
    {
    \begin{tabularx}{0.92\linewidth}{p{1.4cm}<{\centering}p{1.4cm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{1.0mm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{1.0mm}<{\centering}p{1.0cm}<{\centering}p{1.0mm}<{\centering}p{1.0cm}<{\centering}p{1.0mm}}
        \TableAblationAttn
    \end{tabularx}
    }
    \end{center}
    }
    \end{minipage}
    }
    \\
    \vspace{1.5em}
    
    \label{tab:ablations} \vspace{-2.0em}
\end{table*}
